AFLNet Five Years Later: On Coverage-Guided Protocol Fuzzing

Protocol implementations are stateful which makes them difficult to test: Sending the same test input message twice might yield a different response every time. Our proposal to consider a sequence of messages as a seed for coverage-directed greybox fuzzing, to associate each message with the corresponding protocol state, and to maximize the coverage of both the state space and the code was first published in 2020 in a short tool demonstration paper. AFLNet was the first code- and state-coverage-guided protocol fuzzer; it used the response code as an indicator of the current protocol state. Over the past five years, the tool paper has gathered hundreds of citations, the code repository was forked almost 200 times and has seen over thirty pull requests from practitioners and researchers, and our initial proposal has been improved upon in many significant ways. In this paper, we first provide an extended discussion and a full empirical evaluation of the technical contributions of AFLNet and then reflect on the impact that our approach and our tool had in the past five years, on both the research and the practice of protocol fuzzing.

==> sections/abstract.tex <==

Greybox fuzzing is the most widely used technique for finding vulnerabilities in software systems. At compile time, artifacts of interest are instrumented. At run-time during the test executions in the fuzz campaign, the frequency of occurrence of the instrumented artifacts constitute a feedback from the current test executions. The feedback function is then used to determine next test executions, based on random mutations of the current program inputs. In this paper, we present \aflnet a greybox fuzzer for network protocol implementations. Such implementations tend to be stateful in nature, and yet the underlying state machine(s) capturing the software behavior are often not available. \aflnet tackles stateful systems by capturing the system output as a proxy of the system state and using it to drive future test executions in the fuzz campaign. Extensive experiments on the ProFuzzBench dataset for protocols show the high effectiveness of our state feedback in guiding the fuzz campaign. The \aflnet tool and all experimental artifacts are available open source for usage by researchers and practitioners.
